Partial Transportability for Domain Generalization

A fundamental task in AI is providing performance guarantees for predictions made in unseen domains. In practice, there can be substantial uncertainty about the distribution of new data, and corresponding variability in the performance of existing predictors. Building on the theory of partial identification and transportability, this paper introduces new results for bounding the value of a functional of the target distribution, such as the generalization error of a classifier, given data from source domains and assumptions about the data generating mechanisms, encoded in causal diagrams. Our contribution is to provide the first general estimation technique for transportability problems, adapting existing parameterization schemes such Neural Causal Models to encode the structural constraints necessary for cross-population inference. We demonstrate the expressiveness and consistency of this procedure and further propose a gradient-based optimization scheme for making scalable inferences in practice. Our results are corroborated with experiments.

==> 07_odds_ratio.tex <==
\subsection{Bounded odds ratio}
For un-identifiable factors such as $Q_{\M^*}[W,Y]$, evaluating bounds requires a search over the set of all possible SCMs $\3M$. This is generally not feasible, as there is no constraint on the corresponding mechanisms $\1F$ and distributions $P(\U)$ in the target domain $\M^*$. Instead, we assume that their possible deviation across domains could be specified by a user defined factor $\Lambda$ as follows.

\begin{condition}[Bounded odds ratio]
    \label{cond:bounded_odds}
    Given $\G^{\Delta}$ and $\3P$. For any $V\in\Delta$, let $\C_V$ denote the $c$-component containing $V$ in $\G^*$. The $c$-factor $Q_{\M^*}[\C_V]$ does not differ from $Q_{\M^1}[\C_V]$ by more than a factor $\Lambda_{\C_V} \geq 1$, that is,
    \begin{align}
        \label{eq:bounded_odds_ratio}
        \Lambda_{\C_V}^{-1} \leq Q_{\M^*}[\C_V] \hspace{0.1cm}/\hspace{0.1cm} Q_{\M^i}[\C_V] \leq \Lambda_{\C_V},
    \end{align}
    for some $i=1,\dots,k$. This set of inequalities (\Cref{eq:bounded_odds_ratio}) for all is denoted $\3I$. 
\end{condition}

When $\Lambda = 1$, this condition describes the assumption that $c$-factors are unchanged across domains. As $\Lambda \rightarrow \infty$, larger and larger discrepancies are allowed. Under \Cref{cond:bounded_odds}, we formulate a relaxation of the problem in \Cref{eq:problem_formulation},
\begin{align}
    \left(\min_{\1M\in\mathbb M} \1R_\1M, \max_{\1M\in\mathbb M} \1R_\1M \right) \text{ s.t. } P_\1M \text{ is compatible with } \3P \text{ and } \mathfrak{C}.
\end{align}

We now define nuisance functions and estimators for evaluating extrapolation error.

\begin{definition}[Nuisance function]
    \label{def:nuisance_function}
    For a given graph $\G$ and $\Lambda_{\C_V} \geq 1$, let $\mathfrak S:=\mathfrak S(\V)$ denote the decomposition of $P_{\M^*}(\Y, \Z)$ into factors $Q[\cdot]$. Denote $\mathfrak S_{\texttt{l}},\mathfrak S_{\texttt{u}}$ the lower and upper bounds on $\mathfrak S$, respectively, with non-identifiable factors replaced using the bounds given by \Cref{cond:bounded_odds}. Define $\pi_{\texttt{l}}:= \pi_{\texttt{l}}(\V) = \mathfrak S_{\texttt{l}}(\V) / P(\V)$ and $\pi_{\texttt{u}}:= \pi_{\texttt{u}}(\V) = \mathfrak S_{\texttt{u}}(\V) / P(\V)$. 
\end{definition}

\begin{proposition}
    \label{prop:bound_estimator}
    Let $\pi_{\texttt{l}},\pi_{\texttt{u}}$ denote the nuisance functions defined in \Cref{def:nuisance_function}. Assume that $\pi_{\texttt{l}},\pi_{\texttt{u}}$ are well-defined for all $\v$. Then, for any $\y,\z$,
    \begin{align}
        \min_{\1M\in\mathbb M} \mathbb E_P[\Y\mid \x;\M] \geq \3E_P[\pi_{\texttt{l}}(\Y,\x) \Y \mid \x,]
    \end{align}
\end{proposition}

==> A_experiments_app.tex <==
\section{Experiments}
\label{sec:experiments}
This section evaluates credible intervals and the performance of solutions derived from them on two synthetic examples.
For the approximation of bounds and expectations, we draw 5,000 samples from posterior distributions $P(\cdot \mid \bar{\*v})$. Further details, experiments, and all data generating mechanisms are given in \Cref{sec:exp_detail_app}.

\subsection{Example on Smoking and Lung Cancer}
\label{sec:smoking}
This experiment is inspired by the debate around the relationship between smoking and lung cancer in the 1950's \citep{us2014health}. We consider $\3M: \{M^1, M^*\}$ that describe the effect of an individual's smoking status $S$ on lung cancer $C$, including related measured variables such presence of tar in the lungs $T$, and demographic factors $\W$. The data generating mechanism is given by
\begin{align*}
    \M^i = \begin{cases}
        \V &= \{\W,S,T,C\}\\
        \U &= \{\U_W, U_S, U_T, U_{SC}\}\\
        \1F &= \begin{cases}
            f_{W}(u_W) &= u_W, \text{ for } W\in\W, U_W \in \U_W\\
            f_S(\w,u_S, u_{SC}) &= \begin{cases}
                1, &\text{ if } \sum_i w_i/d + u_{SC} + u_S - 2 > 0\\
                0, &\text{ otherwise}
            \end{cases}\\
            f_T(s,u_T) &= \begin{cases}
                1, &\text{ if } s - 0.5u_T - 1 > 0\\
                0, &\text{ otherwise}
            \end{cases}\\
            f_C(\w,u_C, u_{SC}) &= \begin{cases}
                1, &\text{ if } t - \sum_i w_i/d + u_{SC} - 1 > 0\\
                0, &\text{ otherwise}
            \end{cases}\\
        \end{cases}\\
        P(\U) &\text{defined such that } U_S, U_T, U_{SC} \sim Bern(0.5), U_W \sim N(0,1), W\in\W,
    \end{cases}
\end{align*}

The quantity to upper-bound is the target mean squared error: $R_{P^*}(h) := \mathbb{E}_{P^*}[(C - h(\W,S,T))^2]$ of cancer prediction algorithms $f:\supp_\W \times \supp_S \times \supp_T \rightarrow \supp_C$ trained on $\{M^1\}$. We consider the candidate predictors $h(\w,s,t) \in \{\3E_{P^{M^1}}[C],\3E_{P^{M^1}}[C \mid \w, s, t]\}$.


\subsection{Prediction of Alzheimer's disease across hospitals}
\label{sec:app_performance_comaprisons_neurodegenrative}

This experiment considers the design of prediction rules for the development of Alzheimer's disease in a target hospital $M^*$ in which no data could be recorded. Instead, investigators have access to data from two related studies conducted in domains $M^1$ and $M^2$. SCMs $\3M:\{M^1,M^2,M^*\}$ are given as follows,

\begin{align*}
    \M^i = \begin{cases}
        \V &= \{X_1, X_2, W, Y\}\\
        \U &= \{U_{WY}, U_{X_2}, U_{W}, U_{X_1X_2}\}\\
        \1F &= \begin{cases}
            f_{X_1}(U_{X_1X_2}) &= \begin{cases}
                1, &\text{ if } U_{X_1X_2} > 0 \text{ and } i=2,*\\
                1, &\text{ if } U_{X_1X_2} - 0.5 > 0 \text{ and } i=1\\
                0, &\text{ otherwise}
            \end{cases}\\
            f_{X_2}(U_{X_1X_2},U_{X_2}) &= \begin{cases}
                1, &\text{ if } U_{X_1X_2} + U_{X_2}> 0\\
                0, &\text{ otherwise}
            \end{cases}\\
            f_W(X_1,U_{WY},U_W) &= \begin{cases}
                1, &\text{ if } X_1 + U_{WY} +1.5 U_W - 1 > 0 \text{ and } i=*\\
                1, &\text{ if } X_1 + U_{WY} - U_W + 1 > 0 \text{ and } i=1,2\\
                0, &\text{ otherwise}
            \end{cases}\\
            f_Y(W,X_1,U_{WY}) &= \begin{cases}
                1, &\text{ if } W - U_{WY} + 0.1X_1 - 1 > 0\\
                0, &\text{ otherwise}
            \end{cases}\\
        \end{cases}\\
        P(\U) &\text{defined such that } U_{WY}, U_{X_2}, U_{W}, U_{X_1X_2} \sim \1N(0,1),
    \end{cases}
\end{align*}



==> A_old_proofs.tex <==
\section{Proofs}
\label{sec:proofs}

\begin{lemma}
    No proper subset of a domain-independent Markov boundary is a domain-independent Markov boundary.
\end{lemma}

\begin{proof}
    By definition, for every $\*W\in \*Z$ in a domain-independent Markov boundary $\*Z$, $(\*W\notindep Y \mid \*Z \backslash \*W)_{\G^{i,j}}$. A set $\*R$ strictly contained in $\*Z$ cannot be a domain-independent Markov boundary as additional variables $\*Z\backslash\*R$ can be included such that $(\*Z\backslash\*R\notindep Y \mid \*R)_{\G^{i,j}}$ and $(Y\indep \*S \mid \*Z\backslash\*R, \*R)_{\G^{i,j}}$ $i,j=1,\dots,k$ which violates the third condition in the definition of a domain-independent Markov boundary.
\end{proof}
 
\textbf{\Cref{prop:optimal_invariant_predictor} restated.} \textit{Given selection diagrams $\{\G^{i,j}:i,j=1,\dots,k\}$, an optimal invariant predictor is defined as,
\begin{align}
    \underset{f\in \1F_{\text{inv}}}{\text{arg min}} \hspace{0.1cm}\max_{i=1,\dots,k} \mathbb E_{P^i}[(Y - f(\*X))^2],
\end{align}
Such a solution is a function of $\*Z\subseteq\*X$, which is a domain-independent Markov boundary for $Y\in\*V$.}

\begin{proof}
Given selection diagrams $\{\G^{i,j}:i,j=1,\dots,k\}$ the class of invariant predictors $\1F_{\text{inv}}$ is defined as the set of predictors $\mathbb E_{P}[Y\mid \*z]$ where $(Y\indep \*S \mid \*Z)_{\G^{i,j}}$ for $i,j=1,\dots,k$ and the expectation is taken with respect to any $P$ among source domain distributions. The claim is that $\*Z$ must be a domain-independent Markov boundary for $Y$. 

For a contradiction, assume that there exists an optimal invariant predictor that may be written as $\mathbb E_{P^i}[Y \mid \*Z], i=1,\dots,k$, with $\*Z$ not a domain-independent Markov boundary for $Y\in\*V$. Assume that $\*Z$ defines and invariant predictor across source domains. Then, by virtue of $\*Z$ not a domain-independent Markov boundary, either there exists a $W\in \*Z$ such that $(W\indep Y \mid \*Z \backslash W)_{\G^{i,j}}$ for $i,j=1,\dots,k$; or there exists a subset $\*R \subset \*V\backslash\*Z$ such that $(Y\indep \*S \mid \*Z, \*R)_{\G^{i,j}}$ and $(\*R\notindep Y \mid \*Z)_{\G^{i,j}}$ for $i,j=1,\dots,k$. In the former, if $\*Z \backslash W$ is not a domain-independent Markov boundary we can continue removing independent variables from $\*Z \backslash W$ to reach a domain-independent Markov boundary concluding that, essentially, $\mathbb E_{P^i}[Y \mid \*Z]$ is not distinct from an invariant predictor defined conditional on a domain-independent Markov boundary. In the latter, $\*R \subset \*V\backslash\*Z$ could be added to the conditioning set resulting in an improvement of prediction performance as $(\*R\notindep Y \mid \*Z)_{\G^{i,j}}$ while maintaining invariance as $(Y\indep \*S \mid \*Z, \*R)_{\G^{i,j}}$.
\end{proof}

\textbf{\Cref{prop:invariant_predictor_generalization} restated.}
\textit{Given a set of selection diagrams $\{\G^{i,j}:i,j=1,\dots,k\}$, let $\Delta = \bigcup_{i,j} \Delta^{i,j}$ be the set of variables in $\*V$ whose causal mechanisms differ between any two source domains, and let $\*S = \{S_V: V\in\Delta\}$. The optimal invariant predictor is a solution to \Cref{eq:robust_optimization} if selection nodes in all selection diagrams $\{\G^{i,*}:i=1,\dots,k\}$ are given by $\*S$ with edges $\{S_V\rightarrow V\}_{S_V\in\*S}$.}

\begin{proof}
    Given a set of selection diagrams $\{\G^{i,j}:i,j=1,\dots,k\}$, let $\Delta = \bigcup_{i,j} \Delta^{i,j}$ be the set of variables in $\*V$ whose causal mechanisms differ between any two source domains, and let $\*S = \{S_V: V\in\Delta\}$. 
    
    Assume that selection nodes in all selection diagrams $\{\G^{i,*}:i=1,\dots,k\}$ are given by $\*S$ (and with edges $\{S_V\rightarrow V\}_{S_V\in\*S}$). In that case, the optimal invariant predictor, written $\mathbb E_{P^1}[Y \mid \*Z] = \mathbb E_{P^M}[Y \mid \*Z]$ for any $M\in\1M(\G)$. Any additional variable $W$ in the conditioning set is either irrelevant for prediction, i.e. $\mathbb E_{P^M}[Y \mid \*Z] = \mathbb E_{P^M}[Y \mid \*Z, W]$, or breaks the independence between $Y$ and selection nodes, which implies that $\mathbb E_{P^M}[Y \mid \*Z, W]$ varies as a function of $M$. Since the the functional form of $M$ (besides the arguments of functions) are not constrained by selection diagrams, for any fixed prediction function $\mathbb E_{P^M}[Y \mid \*Z, W]$, we can always find a domain $M'\in \1M(\G)$ that makes the error $\mathbb E_{P^{M'}}[(Y - \mathbb E_{P^M}[Y \mid \*Z, W])^2]$ arbitrarily large, and thus higher than $\mathbb E_{P^{M'}}[(Y - \mathbb E_{P^M}[Y \mid \*Z])^2]$ which is fixed for any $M'$.
\end{proof}

\textbf{\Cref{prop:super_structure} restated.} \textit{Let $[l(\*x),u(\*x)]$ be the solution to a partial transportability task with selection diagrams $\{\G^{*,i}: i = 1,\dots,k\}$, and let $[\tilde l(\*x),\tilde u(\*x)]$ be an alternative solution derived with super-structures of $\{\G^{*,i}: i = 1,\dots,k\}$. Then,  $[l(\*x),u(\*x)]\subseteq [\tilde l(\*x),\tilde u(\*x)]$.}

\begin{proof}
    A super-structure $\tilde{\G}$ of a given selection diagram $\G$ either introduces additional selection nodes or introduces additional edges. A super-structure defines a strictly larger class of SCMs $\M(\tilde{\G})$ that subsumes $\M(\G)$, i.e. $\M(\tilde{\G}) \subset \M(\tilde{\G})$, as additional edges or selection nodes expand the functions that parameterize a given variable. In particular, 
    \begin{align}
    \underset{M \in \M(\G)}{\text{min / max}}\hspace{0.1cm} \mathbb E_{P_M}[Y \mid \*x] \subset \underset{M \in \1M(\tilde{\G})}{\text{min / max}} \hspace{0.1cm}\mathbb E_{P_M}[Y \mid \*x].
    \end{align}
\end{proof}

\textbf{\Cref{prop:median_guarantees} restated.}
\textit{Fix $\*x$, and let $[l(\*x),u(\*x)]$ denote the solution to a particular partial transportability task. Then,
\begin{align*}
    \max_{M\in\M(\G^*)} &\mathbb E_{P^M}[(Y - \underset{M \in \M(\G^*)}{\texttt{med}} \mathbb E_{P^M}[Y\mid \*x])^2]\\
    \leq&\max_{M\in\M(\G^*)}\Big(\mathbb E_{P^M}[ (Y - \mathbb E_{P^M}[Y\mid \*x])^2] + \frac{1}{4}\mathbb E_{P^M}[\left(u(\*x)-l(\*x)\right)^2]\Big).
\end{align*}
Under the condition that the irreducible error $\mathbb E_{P^M}[ (Y - \mathbb E_{P^M}[Y\mid \*x])^2]$ is constant across $M\in\1M(\G^*)$, $\texttt{med}_{M \in \M(\G^*)} \mathbb E_{P^M}[Y\mid \*x]$ is a solution to the problem in \Cref{def:causal_robust_optimization}. }
  

\begin{proof}
For a given set of selection diagrams and data, let $[l(\*x),u(\*x)]$ denote the solution of the partial transportability task for the query $\mathbb E_{P^M}[Y\mid \*x], M \in \M(\G^*)$. Then,
\begin{align*}
    &\max_{M\in\M(\G^*)} \mathbb E_{P^M}[(Y - \underset{M \in \M(\G^*)}{\texttt{med}} \mathbb E_{P^M}[Y\mid \*X])^2]\\
    &=\max_{M\in\M(\G^*)}\left(\mathbb E_{P^M}[ \left(Y - \mathbb E_{P^M}[Y\mid \*X] + \mathbb E_{P^M}[Y\mid \*X]- \underset{M \in \M(\G^*)}{\texttt{med}} \mathbb E_{P^M}[Y\mid \*X]\right)^2]\right)\\
    &=\max_{M\in\M(\G^*)}\left(\mathbb E_{P^M}[ (Y - \mathbb E_{P^M}[Y\mid \*X])^2] + \mathbb E_{P^M}[(\mathbb E_{P^M}[Y\mid \*X]- \underset{M \in \M(\G^*)}{\texttt{med}} \mathbb E_{P^M}[Y\mid \*X])^2]\right)\\
    &\leq\max_{M\in\M(\G^*)}\left(\mathbb E_{P^M}[ (Y - \mathbb E_{P^M}[Y\mid \*X])^2] + \frac{1}{4}\mathbb E_{P^M}[\left(u(\*X)-l(\*X)\right)^2]\right).
\end{align*}
The second equality holds because the cross term in the expansion of the square equal 0 as $\mathbb E_{P^M}[(Y - \mathbb E_{P^M}[Y\mid \*X])] = 0$. The inequality holds because the largest distance between $\mathbb E_{P^M}[Y\mid \*X]$ and the median of values $\mathbb E_{P^M}[Y\mid \*X]$ can reach as a function of $M\in\1M(\G^*)$ is half the distance between maximum and minimum values of $\mathbb E_{P^M}[Y\mid \*X]$ across $M\in\1M(\G^*)$, that is $(u(\*X)-l(\*X))/2$.

If $\mathbb E_{P^M}[ (Y - \mathbb E_{P^M}[Y\mid \*X])^2]$ is equal to a constant value independent of $M$, it can be taken out of the maximization and we are left with the optimization problem,
\begin{align}
    \underset{f}{\text{arg min}}\hspace{0.1cm}\max_{M\in\M(\G^*)} \mathbb E_{P^M}[(\mathbb E_{P^M}[Y\mid \*X] - f(\*X))^2]
\end{align}
For any $x$ and any $f$, we can always choose $M$ such that $|\mathbb E_{P^M}[Y\mid \*x] - f(\*x)| \geq |\mathbb E_{P^M}[Y\mid \*x] - \underset{M \in \M(\G^*)}{\texttt{med}} \mathbb E_{P^M}[Y\mid \*x]|$. For example, by choosing $M$ such that $\mathbb E_{P^M}[Y\mid \*x]= \max_{M\in\M(\G^*)} \mathbb E_{P^M}[Y\mid \*x]$ or $\mathbb E_{P^M}[Y\mid \*x]= \min_{M\in\M(\G^*)} \mathbb E_{P^M}[Y\mid \*x]$ depending on what distance is larger. Therefore, $f(\*x):= \underset{M \in \M(\G^*)}{\texttt{med}} \mathbb E_{P^M}[Y\mid \*x]$ minimizes the robust optimization problem.
\end{proof}

\begin{figure*}[t]
\begin{subfigure}[t]{0.3\linewidth}\centering%(d)
  \begin{tikzpicture}[SCM,scale=0.8]
        \node (X1) at (0,0.9) {$X_1$};
        \node (Y) at (0.5,0) {$Y$};
        \node (X2) at (0,-0.9) {$X_2$};
        \node [sel-node, label=left:{\textcolor{cyan}{$S_{X_1}$}}] (S) at (-0.5,0.3) {};
        \node [sel-node, label=left:{\textcolor{cyan}{$S_{X_2}$}}] (Sx2) at (-0.5,-0.3) {};

        \path [->] (X1) edge (Y);
        \path [->] (Y) edge (X2);
        \path [->] (S) edge[color=cyan] (X1);
        \path [->] (Sx2) edge[color=cyan] (X2);
    \end{tikzpicture}
\caption{$\G^{1,2}$}
\label{fig:examples3:b}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.3\linewidth}\centering%(d)
  \begin{tikzpicture}[SCM,scale=0.8]
        \node (X1) at (0,0.9) {$X_1$};
        \node (Y) at (0.5,0) {$Y$};
        \node (X2) at (0,-0.9) {$X_2$};
        \node [sel-node, label=left:{\textcolor{cyan}{$S_{X_1}$}}] (Sx1) at (-0.5,0.3) {};
        \node [sel-node, label=left:{\textcolor{cyan}{$S_{X_2}$}}] (Sx2) at (-0.5,-0.3) {};

        \path [->] (X1) edge (Y);
        \path [->] (Y) edge (X2);
        \path [->] (Sx1) edge[color=cyan] (X1);
        \path [->] (Sx2) edge[color=cyan] (X2);
    \end{tikzpicture}
\caption{$\G^{*,1}$}
\label{fig:examples3:c}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.3\linewidth}\centering%(d)
  \begin{tikzpicture}[SCM,scale=0.8]
        \node (X1) at (0,0.9) {$X_1$};
        \node (Y) at (0.5,0) {$Y$};
        \node (X2) at (0,-0.9) {$X_2$};
        \node [sel-node, label=left:{\textcolor{cyan}{$S_{X_1}$}}] (Sx1) at (-0.5,0.3) {};

        \path [->] (X1) edge (Y);
        \path [->] (Y) edge (X2);
        \path [->] (Sx1) edge[color=cyan] (X1);
    \end{tikzpicture}
\caption{$\G^{*,2}$}
\label{fig:examples3:d}
\end{subfigure}
\hfill
\null
  \caption{Graphs used for the proof of \Cref{prop:stat_partial}.}
  \label{fig:examples3}
\end{figure*}

\textbf{\Cref{prop:stat_partial} restated.}
\textit{In general, invariant predictors may lie outside of the solution of the partial transportability task.}

\begin{proof}
    We consider a variation of the example used in \Cref{sec:invariance_learning}, given in \Cref{fig:examples3}, as a concrete example to show this fact. There, the solution interval reduces to a single value, i.e. $l(\*x) = u(\*x)$, as $\mathbb E_{P^*}[Y \mid x_1,x_2] = \mathbb E_{P^2}[Y \mid x_1,x_2]$. In turn an optimal invariant predictor takes the form $\mathbb E_{P^1}[Y \mid x_1] = \mathbb E_{P^2}[Y \mid x_1]$ which will differ and as a consequence not be included in the bounds defined by the solution to the partial transportability task.
\end{proof}


\textbf{\Cref{thm:tight}, restated.} \textit{In systems of discretely-observed endogenous variables, credible interval $[\hat l_0(\*x), \hat u_0(\*x)]$ contains the solution to the partial transportability task $[l(\*x),u(\*x)]$ for any $n_i$, and coincides with $[l(\*x),u(\*x)]$ as $n_i \rightarrow \infty$, in observable domains $\pi^i$, $i=1,\dots,k$.}

\begin{proof}
Let $\boldsymbol{\Theta}$ denote the collection of parameters $\boldsymbol\xi, \boldsymbol\theta$ of discrete SCMs that generate the observed data from $P^1, P^2, \dots$. We assume that the prior distribution on $\boldsymbol\xi, \boldsymbol\theta$ has positive support over the domain of $\boldsymbol{\Theta}$. That is, the probability density function $\rho(\boldsymbol \xi) > 0$ and $\rho(\boldsymbol \theta) > 0$ for every possible realization of $\boldsymbol\xi, \boldsymbol\theta$. By the definition of $\boldsymbol{\Theta}$, for every pair of parameter $(\boldsymbol\xi, \boldsymbol\theta) \in \boldsymbol{\Theta}$, it must be compatible with the dataset $\bar{\*v}$, i.e., $P(\bar{\*v} \mid \boldsymbol\xi, \boldsymbol\theta) > 0$. Similarly, given that the prior has positive support in $\boldsymbol\Theta$, $P(\boldsymbol\xi, \boldsymbol\theta \mid \bar{\*v}) > 0$.

Note that parameters $(\boldsymbol\xi, \boldsymbol\theta) \in \boldsymbol{\Theta}$ fully determine the optimal bound  $[l, u]$ for $\mathbb E_{P^*}[Y\mid\*x]$. And so this implies that $P(\mathbb E_{P^*}[Y\mid\*x] \in [l,u] \mid \bar{\*v}) > 0$, which by definition of a $100\%$ credible interval means that $\mathbb E_{P^*}[Y\mid\*x] \in [\hat l_0, \hat u_0]$.

Next we show convergence of the posterior by way of convergence of the likelihood of the data given one SCM $M\in\M(\G^*)$. For increasing sample size the posterior will, with increasing probability, be low for any parameter configuration, i.e. for any $(\boldsymbol\xi, \boldsymbol\theta) \notin \boldsymbol{\Theta}$. By the definition of the optimal bounds $[l,u]$ given by the solution to the partial identification task,
\begin{align}
    P(\bar{\*v}\mid l < \mathbb E_{P^*}[Y\mid\*x] < u) \rightarrow_p 1.
\end{align}
Therefore if the prior on parameters $(\boldsymbol \xi, \boldsymbol\theta)$ defining SCMs is non-zero for any $M\in\M(\G)$, also the posterior converges,
\begin{align}
    P(l < \mathbb E_{P^*}[Y\mid\*x] < u\mid\bar{\*v}) \rightarrow_p 1, 
\end{align}
which is the definition credible intervals $[\hat{l}_0,\hat{u}_0]$ as the 0$^{th}$ and 100$^{th}$ quantiles of the posterior distribution which coincide with $[l,u]$ asymptotically. 
\end{proof} 
